DynamicGlue: Epipolar and Time-Informed Data Association in Dynamic Environments using Graph Neural Networks

The assumption of a static environment is common in many geometric computer vision tasks like SLAM but limits their applicability in highly dynamic scenes. Since these tasks rely on identifying point correspondences between input images within the static part of the environment, we propose a graph neural network-based sparse feature matching network designed to perform robust matching under challenging conditions while excluding keypoints on moving objects. We employ a similar scheme of attentional aggregation over graph edges to enhance keypoint representations as state-of-the-art feature-matching networks but augment the graph with epipolar and temporal information and vastly reduce the number of graph edges. Furthermore, we introduce a self-supervised training scheme to extract pseudo labels for image pairs in dynamic environments from exclusively unprocessed visual-inertial data. A series of experiments show the superior performance of our network as it excludes keypoints on moving objects compared to state-of-the-art feature matching networks while still achieving similar results regarding conventional matching metrics. When integrated into a SLAM system, our network significantly improves performance, especially in highly dynamic scenes.

==> figures/ablation_edges/hilti.tex <==
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
5 & 36.61 / 33.47 & 49.78 / 46.20 & 60.43 / 56.69 & 75.55 / 76.55 & 23.50 / 27.00 & 0.36 / 0.66 & 8.28 / 13.71 \\
10 & 37.37 / 33.41 & 50.41 / 46.45 & 61.14 / 57.24 & \textbf{76.73} / \textbf{77.38} & 23.66 / 27.08 & \textbf{0.21} / 0.62 & \textbf{5.31} / \textbf{12.89} \\
20 & \textbf{38.69} / \textbf{35.13} & \textbf{51.93} / \textbf{47.98} & \textbf{62.52} / \textbf{58.46} & 76.03 / 76.88 & \textbf{24.34} / \textbf{27.76} & 0.21 / \textbf{0.61} & 6.17 / 13.01


==> figures/ablation_edges/hilti_wo_val.tex <==
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
5 & 33.47 & 46.20 & 56.69 & 76.55 & 27.00 & 0.66 & 13.71 \\
10 & 33.41 & 46.45 & 57.24 & \textbf{77.38} & 27.08 & 0.62 & \textbf{12.89} \\
20 & \textbf{35.13} & \textbf{47.98} & \textbf{58.46} & 76.88 & \textbf{27.76} & \textbf{0.61} & 13.01


==> figures/ablation_edges/tum.tex <==
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
5 & 66.48 / 68.87 & 76.99 / 79.27 & 83.98 / 86.31 & 93.96 / 94.12 & 20.57 / 20.48 & 0.65 / 1.04 & 16.61 / 10.66 \\
10 & 67.68 / 69.70 & 78.15 / 79.98 & 84.97 / 86.90 & \textbf{94.12} / \textbf{93.87} & 21.13 / 21.22 & \textbf{0.51} / \textbf{0.59} & \textbf{14.11} / \textbf{6.97} \\
20 & \textbf{68.93} / \textbf{71.23} & \textbf{79.15} / \textbf{81.29} & \textbf{85.86} / \textbf{87.92} & 93.34 / 93.11 & \textbf{23.11} / \textbf{23.15} & 0.65 / 0.90 & 17.57 / 11.23


==> figures/ablation_edges/tum_wo_val.tex <==
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
5 & 68.87 & 79.27 & 86.31 & 94.12 & 20.48 & 1.04 & 10.66 \\
10 & 69.70 & 79.98 & 86.90 & \textbf{93.87} & 21.22 & \textbf{0.59} & \textbf{6.97} \\
20 & \textbf{71.23} & \textbf{81.29} & \textbf{87.92} & 93.11 & \textbf{23.15} & 0.90 & 11.23


==> figures/ablation_fixed_ratio.tex <==
\begin{table*}[!b]
    \footnotesize
    \centering
    \def\matchingCellColor{\cellcolor{gray!10}}
    \begin{tabular}{lccccccc}
        \toprule
        Method & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
        \multicolumn{8}{c}{\matchingCellColor \textbf{Hilti-Oxford Dataset~\cite{hilti2022}}} \\ \midrule
        \input{figures/ablation_fixed_ratio/hilti_0.05} \\ \midrule
        \multicolumn{8}{c}{\matchingCellColor \textbf{TUM4Seasons Dataset~\cite{wenzel2020fourseasons}}} \\ \midrule
        \input{figures/ablation_fixed_ratio/tum_0.05} \\ \bottomrule
        \multicolumn{8}{c}{\matchingCellColor \textbf{Self-Recorded In-The-Wild Dataset}} \\ \midrule
        \input{figures/ablation_fixed_ratio/campus_0.05} \\ \bottomrule
    \end{tabular}
    \caption{}
    \label{tab:ablation_fixed_ratio}
\end{table*}


==> figures/ablation_fixed_ratio/campus_0.05.tex <==
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
LightGlue~\cite{Lindenberger2023} & 18.05 & 33.05 & 49.23 & 83.49 & 4.11 & 0.80 & 0.957144 \\
DynamicGlue & 17.65	& 32.31	& 47.31	& 84.77	& 4.15	& 0.39 & 0.541184


==> figures/ablation_fixed_ratio/hilti_0.05.tex <==
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
LightGlue~\cite{Lindenberger2023} & 16.93 & 27.04 & 37.54 & 87.07 & 4.17 & 0.61 & 1.856212 \\
DynamicGlue & 12.40	& 21.29	& 31.54	& 85.42	& 4.04 & 0.37 & 0.972316


==> figures/ablation_fixed_ratio/tum_0.05.tex <==
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
LightGlue~\cite{Lindenberger2023} & 56.12 & 68.85 & 78.17 & 99.33 & 4.86 &0.45 & 2.833887 \\
DynamicGlue & 51.44	& 65.10	& 75.19	& 97.83	& 4.76	& 0.20 & 1.307202


==> figures/ablation_num_edges.tex <==
\begin{table*}[!b]
    \footnotesize
    \centering
    \def\matchingCellColor{\cellcolor{gray!10}}
    \begin{tabular}{lccccccc}
        \toprule
        Number of Edges & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
        \multicolumn{8}{c}{\matchingCellColor \textbf{Hilti-Oxford Dataset~\cite{hilti2022}}} \\ \midrule
        \input{figures/ablation_edges/hilti_wo_val} \\ \midrule
        \multicolumn{8}{c}{\matchingCellColor \textbf{TUM4Seasons Dataset~\cite{wenzel2020fourseasons}}} \\ \midrule
        \input{figures/ablation_edges/tum_wo_val} \\ \bottomrule
    \end{tabular}
    \caption{Ablation study over the number of self and cross-edges. The best results are marked in bold. Using $10$ edges provides comparably good matching performance and the highest robustness against matching moving objects.}
    \label{tab:ablation_num_edges}
\end{table*}


==> figures/matching_metrics/hilti.tex <==
% \begin{tabular}{lccccccc}
% \toprule
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
Mutual NN & 33.01 / 29.62 & 45.34 / 41.58 & 55.87 / 51.81 & 70.79 / 72.73 & 20.94 / 24.33 & 0.72 / 0.84 & 17.80 / 17.53	\\
% SuperGlue~\cite{Sarlin2020}	 & \textbf{42.80} / \textbf{39.57} & \textbf{56.17} / \textbf{52.71} & \textbf{66.57} / \textbf{62.90} & 70.42 / 72.27 & \textbf{33.08} / \textbf{35.82} & 0.81 / 1.09 & 33.57 / 34.01 \\
% LightGlue~\cite{Lindenberger2023} & 42.66 / 39.10 & 55.59 / 52.06 & 65.65 / 62.13 & \textbf{82.76} / \textbf{83.27} & 29.02 / 31.86 & 0.59 / 0.85 & 18.48 / 21.22 \\ \midrule
LightGlue~\cite{Lindenberger2023} & 36.50 / 34.98 & 49.90 / 47.94 & 60.97 / 58.54 & 59.57 / 62.75 & 32.63 / 35.72 &  0.90 / 1.15 & 43.29 / 41.81 \\ \midrule  % self trained with same data
\frameworkname{} - No edge features & 37.54 / 34.15 & 50.63 / 46.93 & 61.31 / 57.49 & 76.05 / 76.87 & 23.73 / 27.19 & 0.33 / 0.67 & 8.86 / 13.96 \\
\frameworkname{} - No time & 37.18 / 33.60 & 50.19 / 46.49 & 60.90 / 57.09 & 75.81 / 77.17 & 23.96 / 27.27 & 0.28 / \textbf{0.61} & 7.03 / 13.22 \\
\frameworkname{} - No pair norm & 37.52 / 33.87 & 50.60 / 46.77 & 61.22 / 57.41 & 76.65 / 77.61 & 23.54 / 26.55 & 0.25 / 0.59 & 6.93 / \textbf{11.76} \\
\frameworkname{} - iterative & 37.99 / 34.27 & 51.20 / 47.22 & 61.88 / 57.80 & 78.71 / 78.82 & 24.51 / 28.03 & 0.33 / 0.70 & 8.86 / 14.59 \\ \midrule
\frameworkname & 37.37 / 33.41 & 50.41 / 46.45 & 61.14 / 57.24 & 76.73 / 77.38 & 23.66 / 27.08 & \textbf{0.21} / 0.62 & \textbf{5.31} / 12.89
% \bottomrule
% \end{tabular}

==> figures/matching_metrics/hilti_only_ablations.tex <==
DG - No edge features & 34.15 & 46.93 & 57.49 & 76.87 & 27.19 & 0.67 & 13.96 \\
DG - No time & 33.60 & 46.49 & 57.09 & 77.17 & 27.27 & 0.61 & 13.22 \\
DG - No pair norm & 33.87 & 46.77 & 57.41 & 77.61 & 26.55 & 0.59 & 11.76 \\
DG - iterative & 34.27 & 47.22 & 57.80 & 78.82 & 28.03 & 0.70 & 14.59 \\ \midrule
\frameworkname & 33.41 & 46.45 & 57.24 & 77.38 & 27.08 & 0.62 & 12.89


==> figures/matching_metrics/hilti_wo_val.tex <==
% \begin{tabular}{lccccccc}
% \toprule
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
Mutual NN & 29.62 & 41.58 & 51.81 & 72.73 & 24.33 & 0.84 & 17.53	\\
% SuperGlue~\cite{Sarlin2020}	 & \textbf{39.57} & \textbf{52.71} & \textbf{62.90} & 72.27 & \textbf{35.82} & 1.09 & 34.01 \\
% LightGlue~\cite{Lindenberger2023} & 39.10 & 52.06 & 62.13 & \textbf{83.27} & 31.86 & 0.85 & 21.22 \\ \midrule
LightGlue~\cite{Lindenberger2023} & 34.98 & 47.94 & 58.54 & 62.75 & 35.72 &  1.15 & 41.81 \\ \midrule  % self trained with same data
DG - No edge features & 34.15 & 46.93 & 57.49 & 76.87 & 27.19 & 0.67 & 13.96 \\
DG - No time & 33.60 & 46.49 & 57.09 & 77.17 & 27.27 & 0.61 & 13.22 \\
DG - No pair norm & 33.87 & 46.77 & 57.41 & 77.61 & 26.55 & \textbf{0.59} & \textbf{11.76} \\
DG - iterative & 34.27 & 47.22 & 57.80 & 78.82 & 28.03 & 0.70 & 14.59 \\ \midrule
\frameworkname & 33.41 & 46.45 & 57.24 & 77.38 & 27.08 & 0.62 & 12.89
% \bottomrule
% \end{tabular}

==> figures/matching_metrics/tum.tex <==
% \begin{tabular}{@{}lccccccc@{}}
% \begin{tabular}{lccccccc}
% \toprule
% & AUC@5\textdegree $\uparrow$ & AUC@10\textdegree $\uparrow$ & AUC@20\textdegree $\uparrow$& P $\uparrow$ & MS $\uparrow$ & M\textsubscript{mov} $\downarrow$ & K\textsubscript{mov} $\downarrow$ \\ \midrule
Mutual NN 	 & 46.32 / 47.78 & 56.70 / 58.75 & 64.59 / 67.45 & 75.61 / 79.38 & 19.02 / 20.48 & 1.33 / 3.77 & 26.31 / 36.78 \\
% SuperGlue~\cite{Sarlin2020} & 53.66 / 52.40 & 64.69 / 63.78 & 72.41 / 72.23 & 73.13 / 73.24 & \textbf{35.85} / \textbf{36.58} & 1.40 / 2.92 & 50.52 / 57.65 \\
% LightGlue~\cite{Lindenberger2023} & 59.49 / 56.20 & 69.75 / 67.08 & 76.98 / 75.16 & 85.92 / 86.34 & 28.30 / 28.73 & 1.46 / 3.57 & 39.21 / 48.64 \\ \midrule
LightGlue~\cite{Lindenberger2023} & 77.11 / 78.84 & 86.73 / 87.60 & 92.29 / 92.69 & 88.95 / 88.88 & 40.26 / 40.17 & 1.25 / 2.68 & 44.89 / 47.11 \\ \midrule % self trained with same data
\frameworkname{} - No edge features & \textbf{67.99} / 70.14 & \textbf{78.41} / 80.43 & \textbf{85.24} / 87.31 & 93.69 / 93.61 & 21.76 / 21.55 & 0.57 / 0.96 & 16.45 / 10.67 \\
\frameworkname{} - No time & 67.06 / 69.66 & 77.68 / 79.97 & 84.68 / 86.95 & 93.41 / 93.14 & 21.90 / 22.11 & 0.65 / 1.04 & 17.33 / 11.78 \\
\frameworkname{} - No pair norm & 66.42 / 69.18 & 77.14 / 79.52 & 84.21 / 86.52 & \textbf{94.84} / \textbf{94.74} & 20.27 / 20.56 & 0.55 / 0.84 & 14.85 / 9.26 \\
\frameworkname{} - iterative & 67.43 / \textbf{70.28} & 77.84 / \textbf{80.58} & 84.68 / \textbf{87.39} & 94.73 / 94.36 & 22.45 / 22.62 & 0.65 / 1.15 & 17.49 / 12.15 \\ \midrule
\frameworkname & 67.68 / 69.70 & 78.15 / 79.98 & 84.97 / 86.90 & 94.12 / 93.87 & 21.13 / 21.22 & \textbf{0.51} / \textbf{0.59} & \textbf{14.11} / \textbf{6.97}
% \bottomrule
% \end{tabular}


==> figures/old/okvis_ate.tex <==
% \begin{table*}
%     \footnotesize
%     \centering
%     \begin{tabular}{lcl|cc|cc}
%     \toprule
%     \multirow{2}{*}{\textbf{Session}} & \multirow{2}{*}{\textbf{Label}} & & \multicolumn{2}{c|}{\textbf{VIO}} & \multicolumn{2}{c}{\textbf{SLAM}} \\
%      & & & \textbf{Okvis2~\cite{Leutenegger2022}} & \textbf{\frameworkname} & \textbf{Okvis2~\cite{Leutenegger2022}} & \textbf{\frameworkname} \\ \midrule
%     recording\_2021-05-10\_19-15-19 & l & & \textbf{1.39} & 1.75 & \textbf{1.02} & 1.15 \\
%     recording\_2021-01-07\_13-12-23 & l & & 11.04 & \textbf{7.71} & \textbf{1.37} & 2.49 \\
%     recording\_2020-04-07\_11-33-45 & m & & 61.81 & \textbf{37.64} & 76.71 & \textbf{33.67} \\
%     recording\_2020-06-12\_10-10-57 & m & & 29.01 & \textbf{13.34} & \textbf{4.98} & 6.20 \\
%     recording\_2021-05-10\_18-32-32 & m & & 5.42 & \textbf{4.86} & 5.12 & \textbf{5.05} \\
%     recording\_2021-01-07\_10-49-45 & h & & 34.82 & \textbf{10.77} & 14.00 & \textbf{12.42} \\ \bottomrule
%     \end{tabular}
%     \caption{Absolute trajectory errors for various sessions of TUM4Seasons~\cite{wenzel2020fourseasons} in comparison to the state-of-the-art SLAM system Okvis2~\cite{Leutenegger2022}. The best results are marked in bold, the degree of dynamics of the session are categorized in l (low), m (medium), and h (high) depending on the number of moving objects in the scene. Our method vastly outperforms the baseline, especially in high dynamic scenarios as well as in the VIO case (29 \% decreased ATE).}
%     \label{tab:okvis_ate}
%     \vspace{-0.2cm}
% \end{table*}

==> figures/runtimes.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth]{media/timing_plot.pdf}
    \caption{Runtime comparison of our framework in comparison to Superglue~\cite{Sarlin2020} and LightGlue~\cite{Lindenberger2023}.}
    \label{fig:runtimes}
\end{figure}

==> media/sequence.tex <==
\begin{figure}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/Own/session_2/365.png}
    \end{subfigure}   
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/Own/session_2/455.png}
    \end{subfigure}   
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/Own/session_2/515.png}
    \end{subfigure}     
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/Own/session_2/630.png}
    \end{subfigure}     
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/Own/session_2/835.png}
    \end{subfigure}     
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/Own/session_2/925.png}
    \end{subfigure}     
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/Own/session_2/960.png}
    \end{subfigure}   
    \hfill
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/LightGlue/session_2/365.png}
    \end{subfigure}   
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/LightGlue/session_2/455.png}
    \end{subfigure}   
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/LightGlue/session_2/515.png}
    \end{subfigure}     
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/LightGlue/session_2/630.png}
    \end{subfigure}     
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/LightGlue/session_2/835.png}
    \end{subfigure}     
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/LightGlue/session_2/925.png}
    \end{subfigure}     
    \hspace{0cm}
    \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Thesis/figures/match_videos/campus/LightGlue/session_2/960.png}
    \end{subfigure}   
    \caption{Match Sequence Campus}
    \label{fig:match_seq_campus}
\end{figure}    
